Model Synthesis for Communication Traces of System-on-Chip Designs

Concise and abstract models of system-level behaviors are invaluable in design analysis, testing, and validation. In this paper, we consider the problem of inferring models from communication traces of system-on-chip~(SoC) designs. The traces capture communications among different blocks of a SoC design in terms of messages exchanged. The extracted models characterize the system-level communication protocols governing how blocks exchange messages, and coordinate with each other to realize various system functions. In this paper, the above problem is formulated as a constraint satisfaction problem, which is then fed to a SMT solver. The solutions returned by the SMT solver are used to extract the models that accept the input traces. In the experiments, we demonstrate the proposed approach with traces collected from a transaction-level simulation model of a multicore SoC design and traces of a more detailed multicore SoC design developed in GEM5 environment.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> discussion.tex <==
\section{Discussions}
\label{sec:discussions}

In this section, we discuss a few observations and insights about \emph{FlowMiner} gained from experiments.

\smallskip
\noindent{\bf Mining Complex Patterns.} 
\emph{FlowMiner} can discover strong temporal relations among messages observed in a set of traces. It uses $100\%$ forward and backward confidence to mine assertions which hold over all traces.
%as we are interested in mining message flows implemented in SoC communication fabrics. 
The analysis of experimental results indicates that these two confidence measures, used together, allow flows with branching structures to be fully extracted from traces if those flows do not share common messages in their specifications. 

On the other hand, if multiple flows with branching structures and common messages are executed, then branches of those flows may not be completely mined.  One example includes two flows as shown in Figure~\ref{fig:ex} such that one is memory write for {\tt CPU\_0} ({\tt x=0}), while the other is memory write for {\tt CPU\_1} ({\tt x=1}).  These two flows share messages $m_5$ and $m_6$ for memory access.  The pattern $(m_3, m_4)$ may not be mined by \emph{FlowMiner} even though $(m_4,m_5,m_6, m_7)$ can be extracted.  This prevents the whole flow in Figure~\ref{fig:ex} from being found.  A typical technique for mining more patterns including those branching ones is to lower the confidence level.  Its drawback is the rapid increase in the total number of mined patterns, majority of which are invalid. %Additionally, finding a confidence level that balances the numbers of valid and invalid patterns can be tricky.  
In this work, we focus on developing the pattern chaining techniques instead of manipulating confidence levels.

\smallskip
\noindent{\bf Invalid Patterns.} Mining excessively large number of invalid patterns is a serious issue to limit specification mining in practical use.  The main reason for mining invalid patterns is the incorrect correlations among messages in traces. \emph{FlowMiner} uses address-based trace slicing and structural causality to exclude incorrect correlations from mining in a certain degree.  More such techniques would be beneficial to improving mining precision.    

%This bias is causing some patterns to be lost. Especially the scenario 4 in \ref{branching} is the type of flows that are out of scope of this tool. This is highly complex shared resources scenario. We call them branching in the flows. For example, two possible branches for this particular flow in Figure~\ref{fig:ex}: one from $t_1$ and another from $t_3$. $FlowMiner$ will search for assertions throughout the trace database. Here, $t_1$ can lead to $t_2$ or $t_10$. And $t_3$ can lead to $t_4$ or $t-9$. If $t_2$ has resulted from $t_1$ alone, then this branch ($t_1, t_2$) will have backward confidence of 100\%, thus will be extracted as an assertion. Similar resolution for $(t_1,t_10), (t_3, t_4)$ and $(t_3, t_9)$. On the other hand, if $t_2$ is also a branch of transition $t_x$, and $t_x$ has another branch $t_y$, then only forward and backward confidence are not enough to find these branches. Because $t_2$ is no more an assertion for transitions $t_1$ and $t_x$ in this extended scenario. To address such scenarios, we proposed mining for longer patterns(assertions). For example, if ($t_x,t_2$) is continually resulting to another set of transitions($t_a,t_b$), then ($t_x,t_2, t_a,t_b$) will constitute an assertion too, thus will be extracted.

%At this stage this tool is good at finding patterns that has many suffixes one prefix or vice versa. But if the SoC implements flows that bundles many suffixes, many prefixes ground truth together, $FlowMiner$ is not a good choice for them. 

\smallskip
\noindent{\bf Traces for Mining.} 
\emph{FlowMiner} can take any number of traces of different lengths provided as input for mining.  More patterns would be mined from longer traces as those traces may include more information about different flow executions.  The number of input traces can have an impact on mining precision as indicated in Section~\ref{sec:mining}.  Since temporal relations among messages extracted from traces are used approximate the causality relations, more input traces with diverse temporal orderings of flow executions can help to eliminate temporal relations that do not hold for all traces, thus reducing the number of invalid patterns to be mined.  

This work considers lossless traces, \ie~all messages of executed flows are captured in traces.  To deal with traces with missing messages,  we can lower the confidence levels.  The side effects of that approach are explained above.  Since \emph{FlowMiner} mines assertions, the patterns that involves missing messages cannot be mined.  In simulation environment, we think this may not be an issue.  A message can be missing due to 1) a design bug, or 2) incorrect instrumentation.  In the former case, a message may be missing only in a few spots in a trace.  On the other hand, a message will be always missing if the instrumentation for observation is set up incorrectly.  When the mining results are returned to the user for examination, the user can query the database of the mined patterns to filter out patterns that are deemed invalid, and to search for patterns that are expected to hold.  If an expected pattern is not included, it signals a problem in the simulation environment.  According to the above observation, the confidence levels of the sequence for a missing pattern can reveal the potential cause. If confidence levels of a missing pattern\footnote{A missing pattern refers to a sequence that is supposed to be pattern but is not mined due to missing messages.} are higher than 0, it is likely caused by a design bug.  Otherwise, incorrect instrumentation would be a more likely problem. 
 
%That means, if only a single transition out of millions traces misses a single event of a flow instance, this instance will not be treated as an assertion, thus won't be extracted.\\

% Should show runtime in results section.
%\textbf{Mining Time:} $FlowMiner$ is a rule based tool. It scans all the traces available. So mining time is proportional to number of traces to be scanned for assertions.


